Protocols for Learning Classifiers on Distributed Data

We consider the problem of learning classifiers for labeled data that has been distributed across several nodes. Our goal is to find a single classifier, with small approximation error, across all datasets while minimizing the communication between nodes. This setting models real-world communication bottlenecks in the processing of massive distributed datasets. We present several very general sampling-based solutions as well as some two-way protocols which have a provable exponential speed-up over any one-way protocol. We focus on core problems for noiseless data distributed across two or more nodes. The techniques we introduce are reminiscent of active learning, but rather than actively probing labels, nodes actively communicate with each other, each node simultaneously learning the important data from another node.

==> new-lin-sep-proof.tex <==
%===============================================================================================
\section{\emph{Two-way} Two-Party Protocols for Linear Separators}
%\section{Linear Separators}
\label{app-sec:linsep}
%\vspace{-0.25cm}
%In this section, we present a detailed description of the two-party two-way protocol for computing an $\eps$-error linear separator in two dimensions.  We also rigorously prove an $O(\log (1/\eps))$ bound on communication required.  
%In order to make the presentation as easy as possible, we repeat some aspects presented in Section \ref{sec:linsep} so this section is more self-contained.  
%First, we present the algorithm for the case of two dimensions and subsequently generalize to higher dimensions.


%-----------------------------------------------------------------------------------------------
%\paragraph{Algorithm overview.}
%The algorithm proceeds in rounds. In each round both nodes send a constant number of points to the other.  The goal is to limit the number of rounds to $O(\log(1/\eps))$ resulting in a total communication complexity of $O(\log(1/\eps))$.  At the end of $O(\log(1/\eps))$ rounds of communication, the algorithm yields a combined classifier $h_{AB}$ that has $\eps$ error on $D$.

%In order to bound the number of rounds, each node must maintain information about which points the \emph{other node} might be classifying correctly or not at any stage of the algorithm. Specifically, suppose $A$ is sent a classifier $h_B$ from $B$ (learned on $D_B$ and hence has zero error on $D_B$) and this classifier misclassifies some points in $D_A$. We denote these points as the  \emph{Set of Disagreement} (\sod) where \sod $ \subseteq D_A$. The remaining points in $D_A$ can be divided into the \emph{Set of Total Agreement} (\sota), which are the points on which classifiers from $A$ and $B$ will continue to agree on in the future, and the \emph{Set of Luck} (\sol), which are points on which the two nodes currently agree, but might disagree later on. The set of disagreement and the set of luck together form the \emph{Set of Uncertainty} $\sou = \sod \cup \sol$, representing all points that may or may not be classified incorrectly by $B$ in the future. 

%Our goal will be to show that the \sou decreases in cardinality by a constant factor in each round. Achieving this will guarantee that at the end of $\log(1/\eps)$ rounds, the size of the \sou will be at most an $\eps$-fraction of the total input. Since $|\sou| \ge |\sod|$, we obtain the desired $\eps$-error classifier. 

%The simplest strategy would be for each node to build a max-margin classifier on all points it has seen thus
%far, and send the support points for this classifier to the other node. This simple protocol might
%converge quickly in practice (we actually compare against it in Section \ref{sec:expts}, it is called \supo,
%		and it often does). However, in principal this protocol may take a linear number of rounds to converge.
%In particular, we show examples in Section~\ref{ssec:kparty-res} where error of \supo increases for difficult
%datasets. Thus, our proposed \oalgo will choose non-max-margin support vectors, but we will show that by sending these points we can achieve provable error and communication trade-off bounds. 
 

% In order to obtain an $\eps$-optimal classifier in $O(\log(1/\eps))$ rounds, the goal at the end of each communication round is to decrease the size of $U_i$ by a constant fraction. The communication stops in the $i^{th}$ round if $\eps |D_A| \geq |\sod|$.  Since $|U_i| \geq |\sod|$ we show that $i$ is always upper bounded by $O(\log(1/\eps))$.
% They basic idea is for $A$ and $B$ to sent the support vectors of all points they have seen so far.  In general, we expect this simple protocol to converge quickly in practice on most realistic data, but we can also show that on adversarial data it may require sending all points.  So our described protocol augments these support vectors with a constant number of additional points which ensure the algorithm with \emph{provably} achieve the desired results even on adversarial data.  



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{The Algorithm}
%\paragraph{Definitions and notation.}
%
%Let $\c{P}^+_A$ and $\c{P}^-_A$ denote polytopes that contain positive and negative points in $D_A$, respectively.  
%Let $\c{C}^+_A$ and $\c{C}^-_A$ denote the convex hulls formed by the positive and negative \sota in $D_A$ after the $i^{\text{th}}$ round, respectively.  
%%We'll denote the convex hull of a set $X$ as $\c{C}(X)$.  
%In general, when sets have a $+$ or $-$ superscript it will denote the restriction of that set to only positive or negative points, respectively.  When clear we will drop the superscript to simplify notation and refer to either set.  
%%For instance, we will use $\c{P}_A$ and $C_{A,i}$, to refer to either one of the polytopes.  
%We denote the \emph{region of uncertainty} $\c{U}_A$ as $\c{P}_A \setminus \c{C}_A$, and note $U_A = \c{U}_A \cap D_A$.  


%In each round $A$ will send to $B$ a set $S_A \subset D_A$, and then $B$ will either terminate with an $\eps$-error classifier $h_B$, or symmetrically return a set of points $S_B \subset D_B$.  
%The points $S_A$ will imply a max-margin classifier $h_A$ on $S_A$ that has $0$ error on $D_A$.  
%will send in reply a set $S_{B,i} \subset D_B$.  
%Let $W_{B,i} = \bigcup_{j=1}^i S_{B,i}$ and $W_{A,i} = \bigcup_{j=1}^i S_{A,i}$ to refer to the union of all points set up through the $i$th round.  
%The set $S_{A,i}$ will include two parts: the support vectors of $D_A \cup W_{B,i-1}$ (except points already in $W_{A,i-1}$) and some additional points described below.  
%The support vectors in $S_{A,i}$ imply a max-margin classifier $h_{A,i}$ (and similar $h_{B,i}$).  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{Early termination.}
%
%Under certain \emph{early-termination} conditions, player $B$ may terminate the protocol and return a valid classifier, even if $h_A$ has more than $\eps$ error on $D_B$.  Any classifier that is parallel to $h_A$ and is shifted less than the margin of the max-margin classifier also has $0$ error on $D_A$.  Thus if any such classifier has at most $\eps$-error on $D_B$, player $B$ can terminate the algorithm and return that classifier.  

%%\begin{wrapfigure}{r}{.5\textwidth}
%\begin{figure}[!htbp]
%\centering %\vspace{-.15in}
%\includegraphics[width=\columnwidth]{figures/early-termination.pdf}
%\label{app-fig:early-term}
%\end{figure}
%%\end{wrapfigure}
%%\vspace{-.15in}
%
%This early-termination observation is important because it allows $B$ to send to $A$ information regarding a $0$-error classifier, with respect to $h_A$, and the points $S_A$ that define it.  
%If $B$ cannot terminate, then either some point in $D_B$ must be completely misclassified by all separators within the margin, or some negative point in $D_B$ and some positive point in $D_B$ must both be in the margin and cannot be separated.  Either scenario implies that any $\eps$-error classifier on $D_B$ must rotate in some direction (either clockwise or counter-clockwise) relative to $h_A$.  
%This is important, because it informs $A$ that all points on $\partial \c{P}_A$ (the boundary of $\c{P}_A$) in the clockwise (resp. counter-clockwise) direction from $S_A$ will never be misclassified by $B$ if $h_B$ rotates in the counterclockwise (resp. clockwise) direction from $h_A$.
This logic will be formalized in Lemma \ref{app-lem:dir-choice}.  

%If the set $S_A$ always has half of $U_A$ on either side, then this process will terminate in at most $O(\log(1/\eps))$ rounds.  But, it may have no points on one side, and always be forced to rotate towards the other side.  
%%\jeff{Perhaps claim we can actually construct such an example.}  
%Thus, the set $S_A$ is chosen judiciously to ensure that $|U_A|$ decreases by at least half each round.  

































%	\begin{lemma}
%		\label{lem:chull-init}
%		There always exists a set of points in $D_A$ that seed the initial convex hull $C_{A,3}$.
%	\end{lemma}

%	\begin{lemma}
%		\label{lem:chull}
%		At any given round $i$, the convex hull $C_{A,i}$ of the points 
%		$(\bigcup_{odd j} (S_{A,j} \cup Z_j) \cup \bigcup_{even k} S_{B,k})$ defines the Set Of Total Agreement.
%	\end{lemma}

%	\begin{lemma}
%		\label{app-lem:split}
%		At any given round $i$, \spl partitions $U_{A,i}$ such that $|U_{A,i+1}| \leq \frac{1}{2}|U_{A,i}|$.
%	\end{lemma}

%	\begin{lemma}
%		\label{lem:dp-bound}
%		The number of data points communicated at each round of \linsep is bounded by	$O(d)$.
%	\end{lemma}

%	\begin{lemma}
%		\label{lem:round-bound}
%		The number of communication rounds for \linsep is	bounded by $O(\log(\frac{1}{\eps}))$.
%	\end{lemma}

%	Combining Lemma~\ref{lem:dp-bound} and Lemma~\ref{lem:round-bound} we obtain the following 
%	Theorem~\ref{th:comm-linsep}.
%	\begin{theorem}
%		\label{th:comm-linsep}
%		For adversarial distributions, the communication complexity of linear separators in two dimensions is
%		$O(d\log(\frac{1}{\eps}))$.
%	\end{theorem}

%	\begin{corollary}
%		\label{cor:pos-polytope}
%		(remark: A statement on what happens when we consider the same for the positive polytope.)
%	\end{corollary}

%	\begin{corollary}
%		\label{cor:ddim}
%		(remark: A statement on the communication complexity for $d$-dimensions.)
%	\end{corollary}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "2011nips-main"
%%% End: 

